A Proof-Generating C Code Generator for ACL2 Based on a Shallow Embedding of C in ACL2

This paper describes a C code generator for ACL2 that recognizes ACL2 representations of C constructs, according to a shallow embedding of C in ACL2, and translates those representations to the represented C constructs. The code generator also generates ACL2 theorems asserting the correctness of the C code with respect to the ACL2 code. The code generator currently supports a limited but growing subset of C that already suffices for some interesting programs. This paper also offers a general perspective on language embedding and code generation.

==> eptcsdata.tex <==
\providecommand{\firstpage}{185}
\providecommand{\publicationstatus}{Rob Sumners, Cuong Chau (Eds.): 17th ACL2 Workshop (ACL2 2022)\\
EPTCS 359, 2022, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.359.15}{10.4204/EPTCS.359.15}}
\pdfoutput=1

